A Holistic Approach to Undesired Content Detection in the Real World

We present a holistic approach to building a robust and useful natural language classification system for real-world content moderation. The success of such a system relies on a chain of carefully designed and executed steps, including the design of content taxonomies and labeling instructions, data quality control, an active learning pipeline to capture rare events, and a variety of methods to make the model robust and to avoid overfitting. Our moderation system is trained to detect a broad set of categories of undesired content, including sexual content, hateful content, violence, self-harm, and harassment. This approach generalizes to a wide range of different content taxonomies and can be used to create high-quality content classifiers that outperform off-the-shelf models.

==> tables/al_exp_1.tex <==
\begin{tabular}{c | c  c}
\toprule
Category & Random Sampling & Active Learning   \\
\midrule
    \w{S} & 0.8724 $\pm$ 0.0073 & \textbf{0.8789} $\pm$ 0.0117 \\
    \w{H} & 0.7650 $\pm$ 0.0138 & \textbf{0.7678} $\pm$ 0.0131  \\
    \w{V} & 0.4991 $\pm$ 0.1429 & \textbf{0.5367} $\pm$ 0.0142 \\
    \w{HR} & \textbf{0.1976} $\pm$ 0.0277 & 0.1884 $\pm$ 0.0530  \\
    \w{SH} & 0.1524 $\pm$ 0.0740 & \textbf{0.2830} $\pm$ 0.0540  \\
    \w{S3} & 0.6742 $\pm$ 0.0690 & \textbf{0.8314} $\pm$ 0.0157  \\
    \w{H2} & 0.7276 $\pm$ 0.0186 & \textbf{0.7681} $\pm$ 0.0167 \\
    \w{V2} & 0.1379 $\pm$ 0.0335 & \textbf{0.3261} $\pm$ 0.0432  \\
\bottomrule
\end{tabular}

==> tables/al_strategies.tex <==
\begin{tabular}{p{2.1cm}c|cccccc}
\toprule
& Category & \multicolumn{2}{c}{Filter bounds} & \% of samples & \multicolumn{2}{c}{Number of samples} \\
& & Lower & Upper & & Stage 2 & Stage 3 \\
\midrule
Random with filtration  
& Sexual & 0.6 & N/A & 3.42\% & 102600 & 1026 \\
& Hate & 0.3 & N/A & 5.5\% & 165000 & 1650  \\
& Violence & 0.2 & N/A & 12.15\% & 364500 & 3645 \\
& Harassment & 0.65 & N/A & 12.15\% & 364500 & 3645 \\
& Self-Harm & 0.1 & N/A & 13.44\% & 403200 & 4032 \\
& S3 & 0.25 & N/A & 4.06\% & 121800 & 1218 \\
& H2 & 0.1 & N/A & 5.5\% & 165000 & 1650 \\
& V2 & 0.1 & N/A & 11.5\% & 345000 & 3450 \\
\midrule
Uncertainty
& Harassment & 0.25 & 0.75 & 8.17\% & 245100 & 2451 \\
& Self-Harm & 0.05 & 0.95 & 8.17\% & 245100 & 2451 \\
& H2 & 0.05 & 0.95 & 3.88\% & 116400 & 1164 \\
& V2 & 0.05 & 0.95 & 8.17\% & 245100 & 2451 \\
\midrule
Random (no filtration)
& N/A & N/A & N/A & 3.89\% & 116700 & 1167 \\
\bottomrule
\end{tabular}
